BackTrack: Robust template update via Backward Tracking of candidate template

Variations of target appearance such as deformations, illumination variance, occlusion, etc., are the major challenges of visual object tracking that negatively impact the performance of a tracker. An effective method to tackle these challenges is template update, which updates the template to reflect the change of appearance in the target object during tracking. However, with template updates, inadequate quality of new templates or inappropriate timing of updates may induce a model drift problem, which severely degrades the tracking performance. Here, we propose BackTrack, a robust and reliable method to quantify the confidence of the candidate template by backward tracking it on the past frames. Based on the confidence score of candidates from BackTrack, we can update the template with a reliable candidate at the right time while rejecting unreliable candidates. BackTrack is a generic template update scheme and is applicable to any template-based trackers. Extensive experiments on various tracking benchmarks verify the effectiveness of BackTrack over existing template update algorithms, as it achieves SOTA performance on various tracking benchmarks.

==> figs/algorithm.tex <==
\begin{algorithm}[H]
\begin{algorithmic}[1]
% \State $\tb{S}=\{s_1, s_2, ... , s_n\}$ is a set of search frames.%\;
% \State $F=\{b_1, f_2, ..., b_n\}$ is a set of predicted bounding boxes.%\;
% \State $\taub$ is a template from current frame.%\;
% \textbf{Initialize :} \\
% \hspace*{\algorithmicindent} $N \gets n$
% \Initialize{$N \gets n$}
% \While{$N > 0$}\\
%       \hspace*{\algorithmicindent}$b_i \gets TRACK(s_i, t)$\\
%       \hspace*{\algorithmicindent}$i_i \gets IOU(y_i, b_i)$\\
%       \hspace*{\algorithmicindent}$N \gets N-1$
% \EndWhile
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \State \tb{s}$_{n}$ is $n$-th search frame.
\State $N$ is a cycle of \algName.
\State $\iouzerothres$ is a threshold for IOU $\sigma_\tvar$.
\ed{\State A$^{thres}$ is an area threshold for early rejection.}
\State $M^{thres}$ is a threshold for count $M$.
% \State 
\State $\tvar:= 1$;  $\tstart:= 1$;  $\tsamprate:= 1$; $M^{thres}:=\lfloor N\iouzerothres\rfloor$ \label{alg:TU:PARAM}
\While{$\tvar \leq $(length of video)}
  \State  $\bbox_\tvar \gets \tracker(\search_\tvar; \template_0,{\template'})$ \Comment{Track forward}
  \If{$MOD(\tvar,N) = 0$
  \tb{and} (Area of $\templatecandi$)$\geq$ A$^{thres}$} \label{alg:TU:ER}
  \State \ed{\Comment{Early rejection}}
    \State $\templatecandi \gets$ Crop($\search_\tvar$,$\bbox_\tvar$)
    \State $M, \sigma_{\tstart} \gets$ {BackTrack}($\templatecandi$, $\tsamprate$, $\tstart$, $\tend\gets\tvar$)
    \If{ ($M \geq M^{thres}$) \&  ($\sigma_{\tstart} \geq \iouzerothres$) } \label{alg:TU:THR}
      \State $\template' \gets \templatecandi$ \Comment{Template update}
      \State $\tstart \gets \tvar$ \Comment{Update \algName~start}
      \State $\tsamprate \gets 1$
    \Else
      \State $\tsamprate \gets \tsamprate+1$
    \EndIf
  \EndIf
  \State  $\tvar \gets \tvar+1$
\EndWhile
 \caption{Template update via \algName}
 \label{alg:TU}
 \end{algorithmic}
\end{algorithm}

\begin{algorithm}[H]
\begin{algorithmic}[1]
\Procedure {$M, \sigma_{\tstart} \gets$ BackTrack} { $\templatecandi$, $\tsamprate$, $\tstart$, $\tend$}
\State $M:=0$;  $\tvar:=\tend$
\While{\tb{TRUE}}
    \State $\tvar \gets \tvar-\tsamprate$ \Comment{Negative means backward}
    \State $\bwdbbox_\tvar$ $\gets$ $\tracker(\search_\tvar; \cdot,\templatecandi)$ \Comment{Track backward}
    \If{ IOU($\bwdbbox_\tvar$,$\bbox_\tvar$) $> 0.5$  } \label{alg:BTC:sigma}
        \State $M \gets M+1$  \Comment{Eq.(\ref{eq:cond2})} \label{alg:BTC:IOU0}%\
    \ed{\Else 
      \State break; \Comment{Early Termination}} \label{alg:BTC:ET} %\; 
    \EndIf
    % \State $M^{Total} \gets M^{total}+1 $
    
    \If{$\tvar=\tstart$} 
        \State break;\Comment{ Ends when arrive to start of Fwd}
    \EndIf
\EndWhile
% \State $\tvar \gets \tstart$%\;
\State $\sigma_{\tstart} \gets $ IOU($\bbox_{\tstart}$, $\bwdbbox_{\tstart}$) \Comment{Eq.(\ref{eq:cond1})}%\;
\EndProcedure
 \caption{Backward tracking algorithm}
\label{alg:BTC}
 \end{algorithmic}

\end{algorithm}







==> figs/graph/archive/moti_stark.tex <==
% \documentclass[12pt,a4paper,onecolumn, openright]{report}
% \usepackage{xcolor}
% \usepackage{pgfplots}
% \usepackage{tikz}

% Define bar chart colors
%
\definecolor{bblue}{HTML}{4F81AA}
\definecolor{rred}{HTML}{C3599A}
\definecolor{ggreen}{HTML}{9BBB90}
\definecolor{ppurple}{HTML}{9F4C7C}


% \begin{document}
\begin{tikzpicture}
    \begin{axis}[
        width  = 6cm, %0.85*\columnwidth,
        height = 3cm,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        bar width=5pt,
        ymajorgrids = true,
        ylabel = {AUC[\%]},
        symbolic x coords={STARK,STARK+Proposed},
        xtick = data,
        scaled y ticks = false,
        enlarge x limits=0.5,
        ymax=73,
        ymin=62,
        extra y ticks=65.8,
        extra y tick labels={}, %STARK w/o TU},
        % extra y tick style={
        %     % in case you should remove the grid from the "normal" ticks ...
        %     ymajorgrids=true,
        %     % ... but don't show an extra tick (line)
        %     ytick style={
        %         /pgfplots/major tick length=0pt,
        %     },
        % }
        % legend cell align=left,
        % legend style={
        %         at={(1,1.05)},
        %         anchor=south east,
        %         column sep=1ex
        % }
    ]
        \addplot[style={bblue,fill=bblue,mark=none}]
            coordinates {(STARK, 64.6) (STARK+Proposed,66.46) };

        \addplot[style={bblue,fill=bblue,mark=none}]
             coordinates {(STARK,65.5) (STARK+Proposed,67.85) };

        \addplot[style={bblue,fill=bblue,mark=none}]
             coordinates {(STARK,65.8) (STARK+Proposed,67.79)};

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {(STARK,66.2) (STARK+Proposed,67.28) };
             
        \addplot[style={ggreen,fill=ggreen,mark=none}]
            coordinates {(STARK, 66.9) (STARK+Proposed,67.33) };

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {(STARK,66.2) (STARK+Proposed,67.79) };

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {(STARK,66.7) (STARK+Proposed,66.76)};

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {(STARK,67.0) (STARK+Proposed,66.29) };

        \legend{No vectorization,TreeScore $>2$,TreeScore $>3$,TreeScore $>4$}
    \legend{}
    \end{axis}
\end{tikzpicture}
% \end{document}

==> figs/graph/archive/moti_stark_hori.tex <==
% \documentclass[12pt,a4paper,onecolumn, openright]{report}
% \usepackage{xcolor}
% \usepackage{pgfplots}
% \usepackage{tikz}

% Define bar chart colors
%
\definecolor{bblue}{HTML}{4F81AA}
\definecolor{rred}{HTML}{C3599A}
\definecolor{ggreen}{HTML}{9BBB90}
\definecolor{ppurple}{HTML}{9F4C7C}


% \begin{document}
\begin{tikzpicture}
    \begin{axis}[
        width  = 6cm, %0.85*\columnwidth,
        height = 3cm,
        major x tick style = transparent,
        ybar=2*\pgflinewidth,
        bar width=3pt,
        ymajorgrids = true,
        ylabel = {AUC[\%]},
        symbolic x coords={STARK,STARK+Proposed},
        xtick = data,
        scaled y ticks = false,
        enlarge x limits=0.5,
        ymax=73,
        ymin=62,
        extra y ticks=65.8,
        extra y tick labels={}, %STARK w/o TU},
        % extra y tick style={
        %     % in case you should remove the grid from the "normal" ticks ...
        %     ymajorgrids=true,
        %     % ... but don't show an extra tick (line)
        %     ytick style={
        %         /pgfplots/major tick length=0pt,
        %     },
        % }
        % legend cell align=left,
        % legend style={
        %         at={(1,1.05)},
        %         anchor=south east,
        %         column sep=1ex
        % }
    ]
    
        \addplot[style={bblue,fill=bblue,mark='*'}]
            coordinates {(5, 64.6) (STARK+Proposed,0) };
        \addplot[style={ggreen,fill=ggreen,mark=none}]
            coordinates {(STARK, 0) (STARK+Proposed,66.46) };
        
        \addplot[style={bblue,fill=bblue,mark=none}]
             coordinates {(STARK,65.5) (STARK+Proposed,67.85) };
        \addplot[style={bblue,fill=bblue,mark=none}]
             coordinates {(STARK,65.5) (STARK+Proposed,67.85) };

        \addplot[style={bblue,fill=bblue,mark=none}]
             coordinates {(STARK,65.8) (STARK+Proposed,67.79)};

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {(STARK,66.2) (STARK+Proposed,67.28) };
             
        \addplot[style={ggreen,fill=ggreen,mark=none}]
            coordinates {(STARK, 66.9) (STARK+Proposed,67.33) };

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {(STARK,66.2) (STARK+Proposed,67.79) };

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {(STARK,66.7) (STARK+Proposed,66.76)};

        \addplot[style={ggreen,fill=ggreen,mark=none}]
             coordinates {(STARK,67.0) (STARK+Proposed,66.29) };

        \legend{No vectorization,TreeScore $>2$,TreeScore $>3$,TreeScore $>4$}
    \legend{}
    \end{axis}
\end{tikzpicture}
% \end{document}

==> figs/graph/archive/motiovation_cycle_bu.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.533333333333333,0.08,0.0823529411764706}
\definecolor{color1}{rgb}{0,1,1}
\definecolor{color2}{rgb}{1,0,1}

\begin{semilogxaxis}[
legend cell align={left},
legend style={fill opacity=1.0, draw opacity=1,text height=4, text opacity=1, at={(0.97,0.01)}, anchor=south east, nodes={scale=0.7, transform shape}},
tick align=outside,
tick pos=left,
title={\(\displaystyle \bf{Success}\)},
x grid style={white!69.0196078431373!black},
xlabel={Cycle of template update, $N$},
xmajorgrids,
xmin=5, xmax=200,
xtick style={color=black},
xtick={5,10,15,20,30,50,100,200},
xticklabels={5,10,15,20,30,50,100,200},
y grid style={white!69.0196078431373!black},
ylabel={AUC [\%]},
ylabel near ticks,
% ymajorgrids,
ymin=60, ymax=75,
ytick style={color=black},
]

\newcommand\markscale{0.8}
\newcommand\markscaletwo{1}
% \newcommand\linethic{ultra thick}
\newcommand\linethic{thick}


% \addplot [mark=*, thick, colorS, dashed]
\addplot [mark=triangle*,mark options={scale=\markscale}, \linethic, colorOB]
table {
5	72.05 
10	72.92
15	73.06
20	72.84
% 25	72.63
30	73.01
50	72.39
100	71.50
200	71.61
};
\addlegendentry{\textbf{OSTrack-\algNameShort}}



\addplot [thick, colorO, densely dotted]
table {%
5	71.1
10	71.1
15	71.1
20	71.1
% 25	71.1
30	71.1
50	71.1
100	71.1
200	71.1
};
\addlegendentry{OSTrack}




\addplot [mark=diamond*,mark options={scale=\markscaletwo}, \linethic, colorMB]
table {%
5	70.1
10	70.2
15	70.3
20	70
% 25	-
30	69.9
50	69.9
100	69
200	69
};
\addlegendentry{MixFormer-\algNameShort}

\addplot [ mark=diamond*,mark options={scale=\markscaletwo}, \linethic, colorMT, densely dashed]
table {%
5	64.4
10	65.6
15	65.9
20	66
% 25	67.1
30	67.5
50	67.5
100	68.1
200	69.2
};
\addlegendentry{MixFormer}



\addplot [thick, colorM,densely dotted]
table {%
5	67.9
10	67.9
15	67.9
20	67.9
% 25	67.9
30	67.9
50	67.9
100	67.9
200	67.9
};
\addlegendentry{MixFormer(w/oTU)}


\addplot [mark=*,mark options={scale=\markscale}, \linethic, colorSB]
table {%
5	66.46
10	67.85
15	67.79
20	67.28
% 25	67.44
30	67.33
50	67.79
100	66.76
200	66.29
};
\addlegendentry{STARK-\algNameShort}


\addplot [mark=*,mark options={scale=\markscale}, \linethic, colorST, densely dashed]
table {%
5	64.6
10	65.5
15	65.8
20	66.2
% 25	62.4
30	66.9
50	66.2
100	66.7
200	67.0
};
\addlegendentry{STARK-ST}

\addplot [thick, colorS, densely dotted]
table {%
5	65.8
10	65.8
15	65.8
20	65.8
25	65.8
30	65.8
50	65.8
100	65.8
200	65.8
};
\addlegendentry{STARK-S}



\end{semilogxaxis}

\end{tikzpicture}


==> figs/graph/archive/motivation_cycle.tex <==
% This file was created by tikzplotlib v0.9.8.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.533333333333333,0.08,0.0823529411764706}
\definecolor{color1}{rgb}{0,1,1}
\definecolor{color2}{rgb}{1,0,1}

\definecolor{bblue}{HTML}{4F81AA}
\definecolor{rred}{HTML}{C3599A}
\definecolor{ggreen}{HTML}{9BBB90}
\definecolor{ppurple}{HTML}{9F4C7C}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=1.0, draw opacity=1,text height=4, text opacity=1, at={(0.97,0.01)}, anchor=south east, nodes={scale=0.7, transform shape}},
tick align=outside,
tick pos=left,
title={\(\displaystyle \bf{Success}\)},
x grid style={white!69.0196078431373!black},
xlabel={Cycle of template update, $N$},
xmajorgrids,
% xmin=0, xmax=205,
xtick style={color=black},
xtick={5,10,15,20,30,50,100,200},
symbolic x coords={5,10,15,20,30,50,100,200},
xticklabels={5,10,15,20,30,50,100,200},
y grid style={white!69.0196078431373!black},
ylabel={AUC [\%]},
ylabel near ticks,
% extra y ticks=65.8,
% extra y tick labels={},
% extra y tick style={
%             ymajorgrids=true,
%             % ... but don't show an extra tick (line)
%             % ytick style={
%             %     /pgfplots/major tick length=0pt,
%             % },
% }
% ymajorgrids,
ymin=62, ymax=70,
ytick style={color=black},
]

\newcommand\markscale{0.8}
\newcommand\markscaletwo{1}
% \newcommand\linethic{ultra thick}
\newcommand\linethic{thick}



% \addplot[ybar] [style={ggreen,fill=ggreen}]
\addplot[ybar] [style={ggreen,fill=ggreen},ultra thick]
%,mark options={scale=\markscale}, \linethic, colorSB]
table {%
5	66.46
10	67.85
15	67.79
20	67.28
% 25	67.44
30	67.33
50	67.79
100	66.76
200	66.29
};
\addlegendentry{STARK-\algNameShort}


% \addplot[ybar] [style={rred}]
\addplot[ybar] [style={rred,fill=bblue},thick]
table {%
5	64.6
10	65.5
15	65.8
};
\addplot[ybar] [style={bblue,fill=bblue}]
table {%
20	66.2
% 25	62.4
30	66.9
50	66.2
100	66.7
200	67.0
};
\addlegendentry{STARK-ST}
\addplot [ultra thick, black, densely dotted]
table {%
5	65.8
10	65.8
15	65.8
20	65.8
% 25	65.8
30	65.8
50	65.8
100	65.8
200	65.8
};
\addlegendentry{STARK-S}



\end{axis}

\end{tikzpicture}


==> figs/table/SOTA_all.tex <==
\begin{tabular}{l|c|ll|ll|ll|lll} 
% \hline
\hlineB{3}
\multirow{2}{*}{Method}  & \multirow{2}{*}{\thead{Template \\ update}} & \multicolumn{2}{c}{LaSOT} & \multicolumn{2}{c}{LaSOT$_{ext}$} & \multicolumn{2}{c}{TrackingNet} & \multicolumn{3}{c}{GOT-10k} \\ 
\cline{3-11}
 & & AUC & $P_{Norm}$ & AUC & $P_{Norm}$ &AUC & $P_{Norm}$ & AO & SR$_{0.5}$ &SR$_{0.75}$ \\ 
\hline
% SiamRPN++ & 49.6 & 56.9 & 34.0 & 41.6 & -- & -- & 51.7 & 61.6 & 32.5 \\
STARK-S &  No & 65.8 & 75.2 &  46.7 & 52.8 & 80.3 & 85.1  & 67.2 &76.1 &61.2\\
STARK-ST & Yes & 66.4\myUpC{0.6} & 76.3\myUpC{1.1}& 47.4\myUpC{0.7} & 53.9\myUpC{1.1} &
81.3\myUpC{1.0} & 86.1\myUpC{1.0} & 68.0\myUpC{0.8} & 77.7\myUpC{1.6} & 62.3\myUpC{1.1} \\
STARK-\algNameShort & Proposed & 67.8\myUpR{2.0} & 78.1\myUpR{2.9} &  49.0\myUpR{2.3} & 55.8\myUpR{3.0} &
81.4\myUpR{1.1} & 86.3\myUpR{1.2} & 69.8\myUpR{2.6} & 80.0\myUpR{3.9} & 64.5\myUpR{3.2} \\
\cline{1-11}
% KeepTrack & 67.1 & 77.2 &  48.2 & - & - & - & - \\
% SwinTrack-B & 69.6 & 78.6 & 47.4 & 57.3 & 71.0 & 80.4 & 68.2 \\
MixFormer &  No & 67.9 & 77.6 &  50.9 & 61.6 & 80.8 & 85.6   & 69.8 & 78.9 & 65.7 \\
MixFormer &  Yes & 69.2\myUpC{1.3} & 78.7\myUpC{1.1} &  51.0\myUpC{0.1} & 61.7\myUpC{0.1} &
83.1\myUpC{2.3} & 88.1\myUpC{2.5}  & 70.7\myUpC{0.9} & 80.0\myUpC{1.1} & 67.8\myUpC{2.1} \\
MixFormer-\algNameShort & Proposed & 70.3\myUpR{2.4} & 80.5\myUpR{2.9} & 52.5\myUpR{1.6} & \tb{63.5}\myUpR{1.9} &
82.8\myUpR{2.0} & 87.9\myUpR{2.3} & 74.8\myUpR{5.0} & 85.0\myUpR{6.1} & 72.6\myUpR{6.9} \\
\cline{1-11}
OSTrack &  No & 71.1 & 81.1 & 50.9 & 58.1 &83.9 &88.5  & 73.7 & 83.2 & 70.8 \\ 
OSTrack-\algNameShort  & Proposed & \tb{73.3}\myUpR{2.2} & \tb{83.7}\myUpR{2.6}&  \tb{53.3}\myUpR{2.4} & 60.6\myUpR{2.5} &
\tb{85.0}\myUpR{1.1} & \tb{89.7}\myUpR{1.2}  & \tb{75.9}\myUpR{2.2} & \tb{86.9}\myUpR{3.7} & \tb{73.3}\myUpR{2.5}\\
\cline{1-11}
% SwinTrack &  No & 71.3 & - & 49.1 & - & 84.0 & 88.2  & 69.4 & 78.0 & 64.3 \\ 
% SwinTrack-\algNameShort  & Proposed & \tb{73.9}\myUpR{2.6} & 83.4\myUpR{-}&  49.9\myUpR{0.8} & -\myUpR{-} &
% 83.7\myUpR{-} & 88.5\myUpR{0.3}  & 70.0\myUpR{0.6} & 78.8\myUpR{0.8} & 65.4\myUpR{1.1}\\
% \hline
\hlineB{3}
\end{tabular}

==> figs/table/motivation_cycle.tex <==
\begin{tabular}{c|c|ll} 
\hline
Index &Update condition &  AUC  & $P_{Norm}$  \\ 
\hline
- & Baseline & 71.1 & 81.1\\
% A & Mean IOU $\geq\sigma^{thres}$  & 72.4\myUpR{1.3} & 82.2\myUpR{1.1}  \\
A & COUNT(IOU$\geq\sigma$) $\geq$ M$^{thres}$    & 72.0\myUpR{0.9} & 81.9\myUpR{0.8}  \\
B & IOU$_{start}$ $\geq \sigma^{thres}$ & 72.8\myUpR{1.7} & 82.7\myUpR{1.6}  \\
% C' & COUNT(IOU\geq\tau) \geq Adaptive P & 71.3\myUpR{2.2} & 80.8\myUpR{2.6}  \\
% D & A \& B & 73.1\myUpR{2.0} & 83.1\myUpR{2.0} & 67.1\\
% E & A \& C & 72.2\myUpR{2.1} & 82.0\myUpR{0.9} & 79.9 \\
% F & B \& C & 73.2\myUpR{2.1} & 83.1\myUpR{2.0}  \\
C & \tb{A \& B} & \tb{73.3}\myUpR{2.2} & \tb{83.7}\myUpR{2.6}  \\
% G & A \& B \& C & 73.2\myUpR{2.1} & 83.2\myUpR{2.4} & 67.0 \\
% +Early rejection  & 73.3\myUpR{2.2} & 83.7\myUpR{2.6}  \\
\hline
\end{tabular}

